Explaining Pre-Trained Language Models with Attribution Scores: An Analysis in Low-Resource Settings

Attribution scores indicate the importance of different input parts and can, thus, explain model behaviour. Currently, prompt-based models are gaining popularity, i.a., due to their easier adaptability in low-resource settings. However, the quality of attribution scores extracted from prompt-based models has not been investigated yet. In this work, we address this topic by analyzing attribution scores extracted from prompt-based models w.r.t. plausibility and faithfulness and comparing them with attribution scores extracted from fine-tuned models and large language models. In contrast to previous work, we introduce training size as another dimension into the analysis. We find that using the prompting paradigm (with either encoder-based or decoder-based models) yields more plausible explanations than fine-tuning the models in low-resource settings and Shapley Value Sampling consistently outperforms attention and Integrated Gradients in terms of leading to more plausible and faithful explanations.

==> agreement.tex <==
%\subsection{Agreement and disagreement analysis}

%\par Following \citet{Krishna2022TheDP}, we analyze the agreement and disagreement of different attribution methods in terms of the plausibility of explanations. We measure this with Pearson correlation, feature agreement and rank agreement. The last two metrics are used in \citet{Krishna2022TheDP}. Details about the metrics and our applications will be provided in the appendix of the final paper. 

%$E_a$ and $E_b$ standing for explanatory signals $a$ and $b$, $n$ standing for length of the explanation, $s$ standing for the complete set of features in the data and $k$ the number of features that are calculated. 

%\textbf{Pearson Correlation}:\\
%\begin{equation}\begin{split}
%r(E_{a}, E_{b})&=\frac{1}{\sqrt{[n\sum_{i=1}^{n} E_{bi}^2 - (\sum_{i=1}^{n} E_{bi})^2]}} \cdot \\[10pt]
%&\frac{\scriptstyle n(\sum_{i=1}^{n} E_{ai} E_{bi})-(\sum_{i=1}^{n} E_{ai})(\sum_{i=1}^{n} E_{bi})}{\sqrt{[n\sum_{i=1}^{n} E_{ai}^2 - (\sum_{i=1}^{n} E_{ai})^2]}} 
%\end{split}
%\end{equation}

%\textbf{Feature Agreement}:\\
%\begin{equation}
%\resizebox{0.91\hsize}{!}{%
%   \text{FA}(E_{a}, E_{b},k)=  \frac{|top\_features(E_a, k) \cap  top\_feature(E_b,k)|}{k} 
%}
%\end{equation}

%\textbf{Rank Agreement}:\\[-15pt]
%\begin{multline}
%\begin{split}
%\resizebox{0.91\hsize}{!}{
%\text{RA}(E_{a}, E_{b},k)=\frac{\scriptstyle\cup_{s\in S}\{s|s\in C_a \land s\in C_b \land s\in C_c\}}{k}\\
%C_a: top\_features(E_a, k)\\
%C_b:top\_features(E_b, k)\\ 
%C_c:rank(E_a,s)=rank(E_b,s)
%}
%\end{multline}

%\par We choose $k$ as the average number of gold tokens in the test set for both data sets, resulting in $k=5$ for TSE and $k=13$ for e-SNLI. Because rank is a stricter method than feature agreement, we decrease $k$ to 2 for both TSE and e-SNLI. Figure \ref{ag_dis} shows the results of different measurements for the two tasks. 

Results are shown in Figure \ref{ag_dis}. The scores are averaged across prompting/fine-tuning methods, training sizes, base models, and model seeds. 

\par We observe that Integrated Gradients and ShapSample have higher correlations than the other comparing pairs for all almost all cases. \citet{Krishna2022TheDP} find that KernelSHAP aligns better with Integrated Gradients than with other gradient-based methods (Gradient, Gradient*Input, SmoothGrad). Our finding complements their conclusions concerning the position of attention on the spectrum.  



